Graph Regularized Encoder Training for Extreme Classification

Deep extreme classification (XC) aims to train an encoder architecture and an accompanying classifier architecture to tag a data point with the most relevant subset of labels from a very large universe of labels. XC applications in ranking, recommendation and tagging routinely encounter tail labels for which the amount of training data is exceedingly small. Graph convolutional networks (GCN) present a convenient but computationally expensive way to leverage task metadata and enhance model accuracies in these settings. This paper formally establishes that in several use cases, the steep computational cost of GCNs is entirely avoidable by replacing GCNs with non-GCN architectures. The paper notices that in these settings, it is much more effective to use graph data to regularize encoder training than to implement a GCN. Based on these insights, an alternative paradigm RAMEN is presented to utilize graph metadata in XC settings that offers significant performance boosts with zero increase in inference computational costs. RAMEN scales to datasets with up to 1M labels and offers prediction accuracy up to 15% higher on benchmark datasets than state of the art methods, including those that use graph metadata to train GCNs. RAMEN also offers 10% higher accuracy over the best baseline on a proprietary recommendation dataset sourced from click logs of a popular search engine. Code for RAMEN will be released publicly.

==> algorithms/train_step.tex <==
\begin{algorithm}
\caption{Bandit ($\cB$)}
\label{alg:bandit}
\begin{algorithmic} 
\REQUIRE $\vw \sim \cN(\mu, 0.1)$
\REQUIRE $i, \cR \leftarrow 0, 0$
\REQUIRE $\vx, \vz$: Document and Label embedding
\STATE $R \leftarrow R + Accuracy(\vx, \vz)$
\STATE $i \leftarrow i + 1$
\IF{$i$ $\%$ $\emph{buffer} == 0$}
\STATE $\Delta \leftarrow \cR - \cR_{p}$
\STATE $\mu \leftarrow \mu + l_r*\Delta/\nabla_{\mu}\log(\cN(\vw\|\mu, 0.1))$
\STATE $\vw \sim \cN(\mu, 0.1)$
\STATE $i \leftarrow 0$
\STATE $\cR_{p} \leftarrow 0.2*\cR + 0.8*\cR_{p}$
\ENDIF
\RETURN $\vw$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Training step}
\label{alg:step}
\begin{algorithmic} 
\REQUIRE $\vX$: Documents in a batch
\REQUIRE $\cG$: Meta-data graphs in the dataset
\STATE $\vZ \sim \vY({\vX})$
\STATE $\vx \leftarrow ENC(\vX)$
\STATE $\vz \leftarrow ENC(\vZ)$
\STATE $\cL \leftarrow Loss(\vx, \vz)*\cB_{xz}(\vx, \vz)$
\FOR{$i \in |\cG|$}
    \STATE $\vN_{x} \sim \cG_{i}({\vX})$
    \STATE $\vn_{x} \leftarrow ENC({\vN_{x}})$
    \STATE $\cL \leftarrow \cL + Loss(\vx, \vn_{x})*\cB_{xi}(\vx, \vz)$
    \STATE $\vN_{z} \sim \cG_{i}({\vZ})$
    \STATE $\vn_{z} \leftarrow ENC({\vN_{z}})$
    \STATE $\cL \leftarrow \cL + Loss(\vz, \vn_{z})*\cB_{zi}(\vx, \vz)$
\ENDFOR
\RETURN $\cL$
\end{algorithmic}
\end{algorithm}

==> figures/dataset_doc_freq.tex <==
Fo\begin{figure}
\centering
\includegraphics[width=0.3\linewidth]{figures/G-LF-WikiSeeAlsoTitles-300K.pdf}
\includegraphics[width=0.3\linewidth]{figures/G-LF-WikiTitles-1M.pdf}
\caption{Label frequency distributions on two benchmark datasets created over Wikipedia articles and Wikipedia categories. The plots show, for each label, the number of train data points tagged with that label. XC applications exhibit extreme label skew wherein 75-90\% of labels are so rare that less than 10-12 data points are tagged with that label. Effective use of metadata becomes essential in such cases where direct supervision is extremely scant. \alg provides a lightweight method to utilize (multiple) label/datapoint graphs to offer superior performance on tail labels with minimal training overhead and no overhead in terms of model size or inference time.}
\label{fig:docfreq}
\end{figure}

==> figures/quantile_plot.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=0.435\textwidth]{figures/sa_quantile_P_5.pdf}~
%     \includegraphics[width=0.45\textwidth]{figures/wt_quantile_P_5.pdf}
%     % \includegraphics[width=0.45\linewidth]{figures/amz_quantile_P_5.pdf}
%     \caption{Quantile wise comparison between \alg and other baselines. \alg gives consistent gains in each quantized bin.}
%     \label{fig:quantile}
% \end{figure}

==> figures/tsne.tex <==
\begin{figure}

    
\end{figure}

==> macros.tex <==
% Standard package includes
\usepackage{times}
\usepackage{latexsym}
% For proper rendering and hyphenation of words containing Latin characters (including in bib files)
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
% \usepackage[finalizecache,cachedir=.]{minted}

% This is not strictly necessary, and may be commented out,
% but it will improve the layout of the manuscript,
% and will typically save some space.
\usepackage{microtype}

% This is also not strictly necessary, and may be commented out.
% However, it will improve the aesthetics of text in
% the typewriter font.
\usepackage{inconsolata}
\usepackage{caption}
\usepackage{listings}
\usepackage{multirow}
\usepackage{soul} % for strikethrough
\usepackage{booktabs}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{graphics}
\usepackage{xspace}
\usepackage{amsmath}
\usepackage{amssymb}  % for checkmarks.
\usepackage{adjustbox}
\usepackage{makecell}
\usepackage{pifont}
\usepackage{tabularx}
\usepackage{xcolor}
\usepackage{tcolorbox}
% \usepackage{fontawesome5}
\usepackage{scalerel,xparse}


\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{xspace}
\usepackage{ulem}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\definecolor{modelgreen}{RGB}{0,204,102}
\definecolor{modelred}{RGB}{255,0,0}
\definecolor{lightgray}{gray}{0.9}


\newcommand{\oursmodel}{\textsc{MoMoS Model}}

\newcommand{\ours}{\textsc{MoMoS}}

\newcommand{\davinci}{{\texttt{text-davinci-003}}\xspace}
\newcommand{\chat}{{\textsc{ChatGPT}}\xspace}
\newcommand{\turbo}{{\texttt{gpt-3.5-turbo}}\xspace}

\newcommand{\cust}{\textsc{Customized}\xspace}



% no indent paragraph.
\newcommand{\niparagraph}[1]{\vspace{1pt}\noindent\textbf{#1}}


\newcommand{\corr}[2]{\textcolor{blue}{\sout{#1} #2}}

\newcommand{\draftonly}[1]{#1}
% Uncomment to hide comments for camera-ready
% \renewcommand{\draftonly}[1]{}

\newcommand{\draftcomment}[1]{\draftonly{#1}}
\newcommand{\review}[1]{\draftcomment{\textcolor{red}{#1}}}

\newcommand{\sid}[1]{\draftcomment{\textcolor{ForestGreen}{Siddarth: #1}}}
\newcommand{\yash}[1]{\textcolor{red}{\textbf{Yash:} #1}}
\newcommand{\bhavyajeet}[1]{\draftcomment{\textcolor{magenta}{Bhavyajeet: #1}}}
\newcommand{\niket}[1]{\draftcomment{\textcolor{purple}{Niket: #1}}}

\newcommand{\todotwo}[1]{\draftcomment{\textcolor{red}{TODO: #1}\xspace}}

% sample tasks
\newcommand{\df}{$\mathbb{DF}$\xspace}

\newcommand{\red}[1]{\textcolor{red}{#1}}

% sample methods
\newcommand{\zshot}{zero-shot\xspace}
\newcommand{\ftune}{fine-tune\xspace}

\usepackage{soul}


\newcommand{\squishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }
\newcommand{\reallysquishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{0.2em} \setlength{\labelwidth}{0.2em}
      \setlength{\labelsep}{0.2em} } }

 \newcommand{\squishend}{
     \end{list} 
 }


\renewcommand{\cite}{\citep}

% colors
\definecolor{ipcolor}{RGB}{61, 133, 198}
\definecolor{modelcolor}{RGB}{241, 194, 50}
\definecolor{opcolor}{RGB}{106, 168, 79}


\definecolor{lightgray}{gray}{0.9}
\definecolor{Box1Color}{RGB}{227, 236, 246}
\definecolor{Box2Color}{RGB}{248, 220, 225}
\definecolor{Box3Color}{RGB}{255, 238, 224}
\definecolor{cbBlue}{RGB}{0, 114, 178}
\definecolor{cbOrange}{RGB}{240, 228, 66}
\definecolor{cbGreen}{RGB}{0, 158, 115}
\definecolor{cbRed}{RGB}{213, 94, 0}
\definecolor{cbPurple}{RGB}{204, 121, 167}
\definecolor{cbSkyBlue}{RGB}{86, 180, 233}
\definecolor{cbGray}{RGB}{128, 128, 128}
% color blind friendly colors
\definecolor{CBF1}{RGB}{255,99,132}  % Red
\definecolor{CBF2}{RGB}{54,162,235}  % Blue
\definecolor{CBF3}{RGB}{255,206,86}  % Yellow
\definecolor{CBF4}{RGB}{75,192,192}  % Green-blue
\definecolor{CBF5}{RGB}{153,102,255} % Purple
\definecolor{CBF1b}{RGB}{205,89,112}  % Darker Red
\definecolor{CBF2b}{RGB}{44,142,215}  % Darker Blue
\definecolor{CBF5b}{RGB}{133,92,225}  % Darker Purple


\definecolor{BoxSkyBlue}{RGB}{149, 200, 216}


\NewDocumentCommand\emojibulb{}{
    \includegraphics[scale=0.1]{figures/idea-bulb.png}
}

% \usepackage{dblfloatfix} % Required to place float across columns
\lstdefinestyle{promptstyle}{
  basicstyle=\ttfamily\scriptsize,
  backgroundcolor=\color{Box1Color},
  frame=single,
  breaklines=true,
  captionpos=b,
  language=,
  tabsize=2
}

\lstset{style=promptstyle}


==> preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{array,url,booktabs,microtype,cite,multirow,hyperref,subcaption,graphicx,mathtools,epstopdf,xspace,amsthm,amsfonts,nicefrac,xcolor,makecell,adjustbox}
\usepackage{wrapfig,lipsum,booktabs}
% \usepackage{algpseudocode}
\RequirePackage[inline,shortlabels]{enumitem}
\setlist{nosep}

% \RequirePackage[color=yellow!10,textsize=scriptsize,linecolor=brown]{todonotes}
% \marginparsep 0pt \marginparwidth 20mm

\makeatletter
\newlength{\eqnsep}
\setlength{\eqnsep}{1pt plus1pt minus.5pt}
\g@addto@macro{\normalsize}{%
\setlength{\abovedisplayskip}{\eqnsep}%
\setlength{\abovedisplayshortskip}{\eqnsep}%
\setlength{\belowdisplayskip}{\eqnsep}%
\setlength{\belowdisplayshortskip}{\eqnsep}}
%\let\c@table\c@figure
\makeatother
\floatsep .8ex plus.2ex minus.1ex
\dbltextfloatsep \floatsep
\textfloatsep \floatsep
\intextsep \floatsep
\newcommand{\ALG}{{RAMEN}\xspace}
\newcommand{\alg}{{RAMEN}\xspace}
% \newcommand{\algtitle}{gRaph regulArization using MEtadata for loNg tail queries}
\newcommand{\algtitle}{Graph Regularized Encoder Training for Extreme Classification}
\makeatletter
\newcommand{\newreptheorem}[2]{\newtheorem*{rep@#1}{\rep@title}
\newenvironment{rep#1}[1]{\def\rep@title{#2 \ref*{##1}}\begin{rep@#1}}{\end{rep@#1}}
}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{thm}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{conj}[thm]{Conjecture}


\newcommand{\init}{\overset{\mathrm{init}}{\leftarrow}}

==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
  %\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  %\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  %\item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:broad_impact}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{app:ethics}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Pelase see Section~\ref{sec:method} and the \suppl}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Please refer to the \suppl}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We have included complete instructions/hyper-parameter settings to reproduce the results. All non-proprietary datasets used in the paper are publicly available \citep{XMLRepo}. Code for \alg will be made available upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please see Section~\ref{sec:exp}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please see Section~\ref{sec:exp}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Please see Section~\ref{sec:results}}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> sections/dataset.tex <==
\section{Dataset}
\label{sec:dataset}
\input{tables/data_stats.tex}

XML Repository~\citep{XMLRepo} provides datasets with various scenarios. However, none of these scenarios involves meta-data graph collected using auxiliary information in the dataset dump. As a result of which two extreme scale graph datasets were created from given data dumps, namely, G-LF-WikiSeeAlsoTitles-300K and G-LF-AmazonTitles-1.6M. These datasets are to be released with the paper for the use of community. 

\textbf{G-LF-WikiSeeAlsoTitles-300K}: Dataset was curated from Wiki dumps \href{https://dumps.wikimedia.org/enwiki/20220520/}{link}. Scenario involved recommending related articles. Articles under ``See Also'' section were used as ground truth predictions. For each article internal hyperlinks and category links were used as meta-data graphs.

\textbf{G-LF-AmazonTitles-1.6M}: Dataset was created using the Amazon dump crawled by~\citep{ni2019}. Scenario involved recommending related products. For a given product, the ``also-buy'' products were used as ground truth. The ``also-view'' and ``similar'' product sections serve as graphs, providing auxiliary signals for the learning process. 

\textbf{Proprietary datasets}: Matching user queries entered on a search engine to advertiser bid keywords is an important problem in any sponsored search pipeline. Any gain in this application, particularly on the long tail of either queries or keywords cam improve the search experience for billions of users while helping small advertisers at the same time. Hence, a toy dataset, G-EPM-1M was created to study the effectiveness of \alg for this application. G-EPM-1M dataset was created by mining the click logs of a popular search engine for a specific time period. The bipartite graph between queries and keywords hence obtained could serve as the base dataset for training any dense retrieval model to predict keywords for a user-entered query. Mining logs obtained the graph for providing auxiliary signals to \alg for three signals: a. Co-session queries: queries that are asked in the same search session by more than one user; b. Co-clicked queries: queries that led to clicks on the same webpage; and c. Co-asked queries: queries that are clicked in the "users also ask" section on the search engine in response to a particular query. All these sources of auxiliary signals were mined for an extended time period.

\textbf{Note}: For each benchmark datasets, test points were removed from the graph nodes. During the evaluations instructions given at XML repository~\citep{XMLRepo} were followed. Please refer to tab.~\ref{tab:data_stats} for dataset statistics.
% \section{Dataset}
% \label{sec:dataset}
% \input{figures/dataset_doc_freq.tex}
% \input{tables/data_stats.tex}

% XML Repository~\citep{XMLRepo} provides datasets with various scenarios. However, none of these scenarios involves meta-data graph collected using auxiliary information in the dataset dump. As a result of which two extreme scale graph datasets were created from given data dumps, namely, G-LF-WikiSeeAlsoTitles-300K and G-LF-AmazonTitles-1.6M. These datasets are to be released with the paper for the use of community. 
% The data creation process for the datasets are explained here:
% \begin{enumerate}
%     \item \textbf{G-LF-WikiSeeAlsoTitles-300K}: The scenario involves recommending related wiki article for a given article. Wikidumps~\href{https://dumps.wikimedia.org/enwiki/20220520/}{link} were crawled and. Only article pages were selected and all other irrelevant meta-information pages were excluded from the dump. In Wikipedia, all pages are interconnected through wikilinks, which serve as the source for constructing the graph. To build the graph from the dump, all the wikilinks present in the articles were utilized. The result was a vast Wikipedia graph, which was filtered to create two separate graphs: one linking article pages to other article pages, and another linking article pages to their corresponding category pages.

%     \item \textbf{G-LF-AmazonTitles-1.6M}
%     The creation of this dataset involved the utilization of raw JSON data dump from \href{http://jmcauley.ucsd.edu/data/amazon/index\_2014.html}{here}. The goal of this dataset is to predict, given a product, the "also-buy" products section present in the raw data dump. The "also-view" and "similar" product sections serve as graphs, providing auxiliary signals for the learning process. 

%     \item \textbf{G-EPM-1M} Matching user queries entered on a search engine to advertiser bid keywords is an important problem in any sponsored search pipeline. Any gain in this application, particularly on the long tail of either queries or keywords cam improve the search experience for billions of users while helping small advertisers at the same time. Hence, a toy dataset, G-EPM-1M was created to study the effectiveness of GRN for this application. G-EPM-1M dataset was created by mining the click logs of a popular search engine for a specific time period. The bipartite graph between queries and keywords hence obtained could serve as the base dataset for training any dense retrieval model to predict keywords for a user-entered query. Mining logs obtained the graph for providing auxiliary signals to GRN for three signals: a. Co-session queries: queries that are asked in the same search session by more than one user; b. Co-clicked queries: queries that led to clicks on the same webpage. Specifically, Simrank++ was performed on a query-webpage click bipartite graph to obtain these edges between queries for the auxiliary graph for GRN; and c. Co-asked queries: queries that are clicked in the "users also ask" section on the search engine in response to a particular query. All these sources of auxiliary signals were mined for an extended time period. The G-EPM-1M dataset hence obtained had around 15M queries and 1M keywords. The auxiliary query-query graph had xx neighbors on average. 

% \end{enumerate}

==> sections/frontmatter.tex <==

\title{\algtitle}

% Authors must not appear in the submitted version. They should be hidden
% as long as the \iclrfinalcopy macro remains commented out below.
% Non-anonymous submissions will be rejected without review.

\author{Antiquus S.~Hippocampus, Natalia Cerebro \& Amelie P. Amygdale \thanks{ Use footnote for providing further information
about author (webpage, alternative address)---\emph{not} for acknowledging
funding agencies.  Funding acknowledgements go at the end of the paper.} \\
Department of Computer Science\\
Cranberry-Lemon University\\
Pittsburgh, PA 15213, USA \\
\texttt{\{hippo,brain,jen\}@cs.cranberry-lemon.edu} \\
\And
Ji Q. Ren \& Yevgeny LeNet \\
Department of Computational Neuroscience \\
University of the Witwatersrand \\
Joburg, South Africa \\
\texttt{\{robot,net\}@wits.ac.za} \\
\AND
Coauthor \\
Affiliation \\
Address \\
\texttt{email}
}


==> tables/ablation_table.tex <==
    



% \begin{table}[h]
%     \centering
%     \caption{Results using Oracle Linker for GCN Vs RAMEN}
%     \label{tab:oracleLinker}
%     \begin{tabular}{l|ccccc}
%     \toprule
% \textbf{Method} & \textbf{P@1}&\textbf{P@5}&\textbf{N@5}&\textbf{PSP@1}&\textbf{PSP@5}\\
% \midrule
% \multicolumn{6}{c}{LF-WikiSeeAlsoTitles-320K}\\ \midrule
% \alg & 35.46 &	18.55 &	36.84 &	28.6 &	34.4\\
% OAK & 33.71 & 17.12 & 34.35 & 25.83 &  30.83\\
% OAK + Oracle & 38.92&19.35&40.35&29.69&34.85\\
% \midrule						
% \multicolumn{6}{c}{LF-WikiTitles-500K}\\ \midrule
% \alg & 48.3	& 19.43	& 36.25	& 28.3	& 26.11\\
% OAK & 44.82 & 17.67 & 33.72 & 25.79 & 24.90\\
% OAK + Oracle & 52.53&24.25&41.98&30.62&32.26\\
% \bottomrule
%     \end{tabular}
% \end{table}


% \begin{table}[h]
%     \centering
%     \caption{Comparison of Training time, prediction time and accuracy of RAMEN 
%  relative to baselines on LF-WikiSeeAlsoTitles-320K dataset.}
%     \label{tab:train_pred_time}
%     \begin{tabular}{l|cccc}
%     \toprule
% \textbf{Method} & \textbf{Train Time} & \textbf{Pred Time} & \textbf{Model size} & \textbf{P@1} \\
% \midrule
% \alg & 1$\times$ & 1$\times$ & 1$\times$ & 35.46 \\
% OAK & 1.5$\times$	& 2$\times$ & 3.5$\times$ &	33.71  \\
% NGAME & 0.87$\times$ & 1$\times$ & 1$\times$ & 32.64   \\
% \bottomrule
%     \end{tabular}
% \end{table}



==> tables/results_eepm.tex <==



==> tables/results_table.tex <==
\begin{table}[!thb]
    \centering
    \caption{Result on short-text benchmark datasets. \alg is up to 15\% more accurate as compared to both text-based and graph-based baselines. RAMEN-M1 indicates accuracies obtained after module M1 i.e. without training the classifier and cross-attention architecture to offer a fair comparison to other methods that do not adopt a classifier. Note that including the classifier and cross-attention architecture offer 2.5 -- 4.5\% improvement in P@1.}
\adjustbox{max width=\linewidth}{  \tabcolsep 3pt
\begin{tabular}{l|cccccc}
\toprule
 & \textbf{PSP@1} & \textbf{PSP@5} & \textbf{P@1} & \textbf{P@5} & \textbf{R@10}  & \textbf{AUC@10} \\
\midrule
\multicolumn{7}{c}{G-LF-WikiSeeAlsoTitles-300K}\\ \midrule						
\alg-M1	 & \textbf{27.99}	 & \textbf{31.78}	 & 39.01	 & 15.19	 & 46.07	 & 48.13\\
NGAME-M1	 & 24	 & 27.34	 & 31.91	 & 12.81	 & 38.34	 & 40.51\\
GraphFormer	 & 15.53	 & 19.87	 & 15.53	 & 8.09	 & 28.61	 & 28.49\\
GraphSage	 & 16.71	 & 27.37	 & 26.13	 & 13.26	 & 38.84	 & -\\
\midrule
\alg	 & 27.83	 & 31.77	 & \textbf{40.5}	 & \textbf{15.86}	 & \textbf{47.88}	 & \textbf{49.73}\\
NGAME	 & 23.25	 & 28.27	 & 33.92	 & 13.86	 & 40.26	 & 42.57\\
ELIAS	 & 14.99	 & 19.45	 & 28.89	 & 12.06	 & 36.95	 & 37.75\\
CascadeXML	 & 12.29	 & 14.49	 & 30.64	 & 11.76	 & 36.5	 & -\\
XR-Transformer	 & 7.9	 & 10.68	 & 15.54	 & 6.93	 & 22.88	 & -\\
ECLARE	 & 21.38	 & 25.5	 & 30.8	 & 13.06	 & 39.04	 & 40.08\\
SiameseXML	 & 23.13	 & 27.35	 & 29.13	 & 12.9	 & 38.45	 & 39.13\\
DECAF	 & 17.79	 & 21.88	 & 28.68	 & 12.16	 & 37.89	 & 38.66\\
Parabel	 & 11.91	 & 14.76	 & 24.36	 & 9.94	 & 30.86	 & 32.67\\
Bonsai	 & 13.26	 & 16.75	 & 25.55	 & 10.56	 & 32.89	 & 34.32\\
\midrule
\multicolumn{7}{c}{G-LF-WikiTitles-1M}\\ \midrule						
\alg-M1	 & \textbf{25.88}	 & 23.09	 & 34.62	 & 14.3	 & 29.8	 & 39.55\\
NGAME-M1	 & 23.69	 & 21.37	 & 31.9	 & 13.52	 & 28.41	 & 37.3\\
GraphFormer	 & 13.97	 & 12.89	 & 16.42	 & 7.92	 & 17.26	 & 28.47\\
GraphSage	 & 21.14	 & 18.79	 & 28.3	 & 11.82	 & 26.21	 & -\\
\midrule
\alg	 & 25.2	 & \textbf{24.33}	 & \textbf{37.79}	 & \textbf{16.76}	 & \textbf{33.43}	 & \textbf{44.36}\\
NGAME	 & 20.01	 & 20.27	 & 32.93	 & 13.99	 & 28.84	 & 38.63\\
ELIAS	 & 17.74	 & 18.77	 & 34.57	 & 15.75	 & 31.11	 & 41.82\\
CascadeXML	 & -	 & -	 & -	 & -	 & -	 & -\\
XR-Transformer	 & -	 & -	 & -	 & -	 & -	 & -\\
ECLARE	 & 18.58	 & 18.24	 & 32.21	 & 14.32	 & 27.56	 & -\\
SiameseXML	 & 20.21	 & 19.79	 & 29.45	 & 13.51	 & 27.01	 & 36.6\\
DECAF	 & 16.21	 & 17	 & 30.88	 & 13.9	 & -	 & -\\
Parabel	 & 14.76	 & 14.98	 & 29.48	 & 13.07	 & 26.19	 & 37.42\\
Bonsai	 & 16.07	 & 16.07	 & 30.19	 & 13.25	 & 26.68	 & 37.75\\
\midrule
\multicolumn{7}{c}{G-LF-AmazonTitles-1M}\\ \midrule						
\alg-M1	 & \textbf{35.23}	 & \textbf{38.56}	 & 41.47	 & 26.86	 & 35.72	 & 49.49\\
NGAME-M1	 & 34.75	 & 37.62	 & 41.34	 & 26.63	 & 35.07	 & 48.89\\
GraphFormer	 & -	 & -	 & -	 & -	 & -	 & -\\
GraphSage	 & -	 & -	 & -	 & -	 & -	 & -\\
\alg	 & -	 & -	 & -	 & -	 & -	 & -\\
NGAME	 & 33.16	 & 38.11	 & \textbf{48.02}	 & \textbf{32.35}	 & \textbf{39.78}	 & \textbf{52.32}\\
ELIAS	 & -	 & -	 & -	 & -	 & -	 & -\\
CascadeXML	 & -	 & -	 & -	 & -	 & -	 & -\\
XR-Transformer	 & -	 & -	 & -	 & -	 & -	 & -\\
ECLARE	 & 27.23	 & 33.3	 & 41.25	 & 28.79	 & 34.59	 & 47.03\\
SiameseXML	 & 29.68	 & 34.16	 & 41.1	 & 28.15	 & 34.55	 & 46.37\\
DECAF	 & 23.83	 & 29.37	 & 39.89	 & 27.61	 & 32.51	 & 44.35\\
Parabel	 & -	 & -	 & -	 & -	 & -	 & -\\
Bonsai	 & -	 & -	 & -	 & -	 & -	 & -\\
\bottomrule
    \end{tabular}
    }  
    \label{tab:results-benchmark}
\end{table}




==> tables/results_table_fulltext_full.tex <==
\begin{table*}[!thb]
    \centering
    \caption{Result on full-text benchmark datasets. \alg is up to 15\% more accurate as compared to both text-based and graph-based baselines. RAMEN-M1 indicates accuracies obtained after module M1 i.e. without training the classifier and cross-attention architecture to offer a fair comparison to other methods that do not adopt a classifier. Note that including the classifier and cross-attention architecture offer up to 6\% improvement in PSP@1 and 4\% improvement in P@1.}
\adjustbox{max width=\linewidth}{  \tabcolsep 3pt
\begin{tabular}{l|cccccccccc}
\toprule
 &  \textbf{PSP@1} &	 \textbf{PSP@3}	&  \textbf{PSP@5}	&  \textbf{PSN@3}	&  \textbf{PSN@5}	&  \textbf{P@1}	&  \textbf{P@3} &	 \textbf{P@5} &	 \textbf{N@3} &	 \textbf{N@5} \\
\midrule
\multicolumn{11}{c}{LF-WikiSeeAlso-320K}\\ \midrule										
\alg-Encoder	 & \textbf{34.38}	 & \textbf{38.22}	 & 41.6	 & \textbf{39.13}	 & 42.02	 & 47.29	 & 31.13	 & 23.37	 & 47.45	 & 49.15\\
NGAME-Encoder	 & 29.6	 & 31.14	 & 32.83	 & 32.56	 & 34.19	 & 45.65	 & 25.04	 & 17.32	 & 44.69	 & 45.43\\
GraphFormer	 & 16.85	 & 18.79	 & 20.98	 & 18.8	 & 20.41	 & 18.14	 & 11.56	 & 8.81	 & 19.28	 & 20.81\\
\alg	 & 33.81	 & 38.17	 & \textbf{41.77}	 & 38.96	 & 41.95	 & \textbf{48.21}	 & \textbf{31.78}	 & \textbf{23.88}	 & \textbf{48.26}	 & \textbf{49.97} \\
NGAME	 & 28.18	 & 30.99	 & 33.33	 & 32.06	 & 34.01	 & 46.4	 & 25.95	 & 18.05	 & 45.83	 & 46.64\\
DEXA	 & 31.81	 & 35.5	 & 38.78	 & 38.94	 & \textbf{78.61}	 & 47.11	 & 30.48	 & 22.71	 & 46.31	 & 47.62\\
CascadeXML	 & 22.26	 & 27.11	 & 31.1	 & 26.21	 & 28.87	 & 40.42	 & 26.55	 & 20.2	 & 39.15	 & 40.55\\
XR-Transformer	 & 25.18	 & 30.13	 & 33.79	 & 29.84	 & 32.59	 & 42.57	 & 28.24	 & 21.3	 & 41.99	 & 43.44\\
PINA	 & -	 & -	 & -	 & -	 & -	 & 44.54	 & 30.11	 & 22.92	 & -	 & -\\
AttentionXML	 & 22.67	 & 26.66	 & 29.83	 & 26.13	 & 28.38	 & 40.5	 & 26.43	 & 19.87	 & 39.13	 & 40.26\\
LightXML	 & 17.85	 & 21.26	 & 24.16	 & 20.81	 & 22.8	 & 34.5	 & 22.31	 & 16.83	 & 33.21	 & 34.24\\
SiameseXML	 & 29.02	 & 32.68	 & 36.03	 & 32.64	 & 35.17	 & 42.16	 & 28.14	 & 21.39	 & 41.79	 & 43.36\\
ECLARE	 & 26.04	 & 30.09	 & 33.01	 & 30.06	 & 32.32	 & 40.58	 & 26.86	 & 20.14	 & 40.05	 & 41.23\\
DECAF	 & 25.72	 & 30.93	 & 34.89	 & 30.69	 & 33.69	 & 41.36	 & 28.04	 & 21.38	 & 41.55	 & 43.32\\
Parabel	 & 17.1	 & 20.73	 & 23.53	 & 20.02	 & 21.88	 & 33.46	 & 22.03	 & 16.61	 & 32.4	 & 33.34\\
Bonsai	 & 18.19	 & 22.35	 & 25.66	 & 21.62	 & 23.84	 & 34.86	 & 23.21	 & 17.66	 & 34.09	 & 35.32\\
\midrule
\multicolumn{11}{c}{LF-Wikipedia-500K}\\ \midrule										
\alg-Encoder	 & 50.94	 & \textbf{58.18}	 & \textbf{61.94}	 & \textbf{57.97}	 & \textbf{61.84}	 & 81.07	 & 63.88	 & 50.1	 & 76.8	 & 75.27\\
NGAME-Encoder	 & \textbf{50.99}	 & 56.02	 & 57.33	 & -	 & -	 & 77.92	 & 54.87	 & 40.95	 & -	 & -\\
GraphFormer	 & 25.16	 & 21.64	 & 21.83	 & 23.64	 & 24.83	 & 31.1	 & 18.63	 & 14	 & 25.26	 & 24.87\\
\alg	 & 43.63	 & 55.98	 & 61.77	 & 54.81	 & 60.15	 & \textbf{85.98}	 & \textbf{67.35}	 & \textbf{52.56}	 & \textbf{81.15}	 & \textbf{79.23} \\
NGAME	 & 41.25	 & 52.57	 & 57.04	 & 51.58	 & 56.11	 & 84.01	 & 64.69	 & 49.97	 & 78.25	 & 75.97\\
DEXA	 & 42.59	 & 53.93	 & 58.33	 & 52.92	 & 57.44	 & 84.92	 & 65.5	 & 50.51	 & 79.18	 & 76.8\\
ELIAS	 & 35.02	 & 45.94	 & 51.13	 & -	 & -	 & 81.26	 & 62.51	 & 48.82	 & 75.12	 & 73.1\\
CascadeXML	 & 31.87	 & 40.86	 & 44.89	 & 40.04	 & 43.87	 & 80.69	 & 60.39	 & 46.25	 & 73.24	 & 70.49\\
XR-Transformer	 & 33.58	 & 42.97	 & 47.81	 & 42.21	 & 46.61	 & 81.62	 & 61.38	 & 47.85	 & 74.46	 & 72.43\\
PINA	 & -	 & -	 & -	 & -	 & -	 & 82.83	 & 63.14	 & 50.11	 & -	 & -\\
AttentionXML	 & 34	 & 44.32	 & 50.15	 & 42.99	 & 47.69	 & 82.73	 & 63.75	 & 50.41	 & 76.56	 & 74.86\\
LightXML	 & 31.99	 & 42	 & 46.53	 & 40.99	 & 45.18	 & 81.59	 & 61.78	 & 47.64	 & 74.73	 & 72.23\\
SiameseXML	 & 33.95	 & 35.46	 & 37.07	 & 36.58	 & 38.93	 & 67.26	 & 44.82	 & 33.73	 & 56.64	 & 54.29\\
ECLARE	 & 31.02	 & 35.39	 & 38.29	 & 35.66	 & 34.5	 & 68.04	 & 46.44	 & 35.74	 & 58.15	 & 56.37\\
Parabel	 & 26.88	 & 31.96	 & 35.26	 & 31.73	 & 34.61	 & 68.7	 & 49.57	 & 38.64	 & 60.51	 & 58.62\\
Bonsai	 & -	 & -	 & -	 & -	 & -	 & 69.2	 & 49.8	 & 38.8	 & -	 & -\\\bottomrule
    \end{tabular}
    }  
    \label{tab:results-benchmark-fulltext}
\end{table*}

==> tables/results_table_shorttext.tex <==
\begin{table*}[!thb]
    \centering
    \caption{Results on short-text benchmark datasets. \alg is up to 15\% more accurate as compared to both text-based and graph-based baselines. RAMEN-M1 indicates accuracies obtained after module M1 i.e. without training the classifier and cross-attention architecture to offer a fair comparison to other methods that do not adopt a classifier. Note that including the classifier and cross-attention architecture offers a 2.5 -- 4.5\% improvement in P@1.}
\adjustbox{max width=\linewidth}{  \tabcolsep 3pt
\begin{tabular}{l|cccccccccc}
\toprule
 &  \textbf{PSP@1} &	 \textbf{PSP@3}	&  \textbf{PSP@5}	&  \textbf{PSN@3}	&  \textbf{PSN@5}	&  \textbf{P@1}	&  \textbf{P@3} &	 \textbf{P@5} &	 \textbf{N@3} &	 \textbf{N@5} \\
\midrule
\multicolumn{11}{c}{LF-WikiSeeAlsoTitles-320K}\\ \midrule	
\alg-M1	 & \textbf{28.99}	 & \textbf{31.79}	 & \textbf{34.54}	 & \textbf{31.7}	 & \textbf{33.62}	 & \textbf{35.24}	 & \textbf{24.03}	 & \textbf{18.37}	 & \textbf{35.25}	 & \textbf{36.47} \\
OAK	 & 25.84	 & 28.51	 & 30.84	 & 28.61	 & 30.34	 & 33.71	 & 22.69	 & 17.12	 & 33.41	 & 34.36\\
GraphSage	 & 21.56	 & 21.84	 & 23.5	 & 22.93	 & 24.57	 & 27.3	 & 17.17	 & 12.96	 & 27.1	 & 28.36\\
GraphFormer	 & 19.24	 & 20.64	 & 22.7	 & 20.98	 & 22.68	 & 21.94	 & 15.1	 & 11.79	 & 22.61	 & 24.02\\
\midrule
\alg	 & \textbf{28.6}	 & \textbf{31.6}	 & \textbf{34.4}	 & \textbf{31.53}	 & \textbf{33.49}	 & \textbf{35.46}	 & \textbf{24.28}	 & \textbf{18.55}	 & \textbf{35.59}	 & \textbf{36.84} \\
NGAME	 & 24.41	 & 27.37	 & 29.87	 & 27.39	 & 29.21	 & 32.64	 & 22	 & 16.6	 & 32.3	 & 33.21\\
DEXA	 & 24.45	 & 26.52	 & 28.62	 & 26.97	 & 28.6	 & 31.71	 & 21.03	 & 15.84	 & 31.34	 & 32.29\\
ELIAS	 & 13.47	 & 15.88	 & 17.69	 & 15.57	 & 16.85	 & 23.36	 & 15.64	 & 11.85	 & 22.86	 & 23.62\\
CascadeXML	 & 12.68	 & 15.37	 & 17.63	 & 14.65	 & 16.05	 & 23.39	 & 15.71	 & 12.06	 & 22.6	 & 23.43\\
XR-Transformer	 & 10.6	 & 11.78	 & 12.72	 & 11.7	 & 12.44	 & 19.44	 & 12.25	 & 8.98	 & 18.26	 & 18.53\\
AttentionXML	 & 9.45	 & 10.63	 & 11.73	 & 10.45	 & 11.24	 & 17.56	 & 11.34	 & 8.52	 & 16.58	 & 17.07\\
SiameseXML	 & 26.82	 & 28.42	 & 30.36	 & 28.74	 & 30.27	 & 31.97	 & 21.43	 & 16.24	 & 31.57	 & 32.59\\
ECLARE	 & 22.01	 & 24.23	 & 26.27	 & 24.46	 & 26.03	 & 29.35	 & 19.83	 & 15.05	 & 29.21	 & 30.2\\
DECAF	 & 16.73	 & 18.99	 & 21.01	 & 19.18	 & 20.75	 & 25.14	 & 16.9	 & 12.86	 & 24.99	 & 25.95\\
Parabel	 & 9.24	 & 10.65	 & 11.8	 & 10.49	 & 11.32	 & 17.68	 & 11.48	 & 8.59	 & 16.96	 & 17.44\\
Bonsai	 & 10.69	 & 12.44	 & 13.79	 & 12.29	 & 13.29	 & 19.31	 & 12.71	 & 9.55	 & 18.74	 & 19.32\\
\midrule
\multicolumn{11}{c}{LF-WikiTitles-500K}\\ \midrule										
\alg-M1	 & \textbf{30.51}	 & \textbf{26.91}	 & \textbf{25.75}	 & \textbf{29.98}	 & \textbf{31.41}	 & \textbf{46.12}	 & \textbf{25.42}	 & \textbf{17.45}	 & \textbf{35.45}	 & \textbf{33.79}\\
OAK 	 & 25.73	 & 25.8	 & 25.01	 & 27.83	 & 29.42	 & 44.84	 & 25.86	 & 17.87	 & 35.42	 & 33.76\\
GraphSage	 & 22.35	 & 19.31	 & 19.15	 & 22.09	 & 23.82	 & 27.19	 & 15.66	 & 11.3	 & 22.6	 & 22.78\\
GraphFormer	 & 22.04	 & 19.2	 & 19.53	 & 21.29	 & 22.78	 & 24.53	 & 14.92	 & 11.33	 & 20.23	 & 20.35\\
\midrule
\alg	 & \textbf{30.06}	 & \textbf{27.41}	 & \textbf{26.44}	 & \textbf{30.22}	 & \textbf{31.74}	 & \textbf{48.24}	 & \textbf{27.41}	 & \textbf{19.02}	 & \textbf{37.64}	 & \textbf{35.86} \\
NGAME	 & 23.12	 & 23.31	 & 23.03	 & 25.34	 & 27.22	 & 39.04	 & 23.1	 & 16.08	 & 31.8	 & 30.75\\
CascadeXML	 & 19.19	 & 19.47	 & 19.75	 & 20.8	 & 22.34	 & 47.29	 & 26.77	 & 19	 & 36.19	 & 34.36\\
AttentionXML	 & 14.8	 & 13.97	 & 13.88	 & 15.24	 & 16.22	 & 40.9	 & 21.55	 & 15.05	 & 29.38	 & 27.45\\
ECLARE	 & 21.58	 & 20.39	 & 19.84	 & 22.39	 & 23.61	 & 44.36	 & 24.29	 & 16.91	 & 33.33	 & 31.46\\
DECAF	 & 19.29	 & 19.82	 & 19.96	 & 21.26	 & 22.95	 & 44.21	 & 24.64	 & 17.36	 & 33.55	 & 31.92\\
Bonsai	 & 16.58	 & 16.34	 & 16.4	 & 17.6	 & 18.85	 & 40.97	 & 22.3	 & 15.66	 & 30.35	 & 28.65\\
\midrule				
\multicolumn{11}{c}{LF-AmazonTitles-1.3M}\\ \midrule			
\alg-M1	 & \textbf{37.02}	 & \textbf{39.95}	 & \textbf{41.22}	 & \textbf{39.3}	 & \textbf{40.48}	 & \textbf{48.7}	 & \textbf{42.88}	 & \textbf{38.36}	 & \textbf{47.28}	 & \textbf{46.26}\\
GraphSage	 & 24.54	 & 24.16	 & 23.72	 & 24.66	 & 24.89	 & 28.13	 & 21.43	 & 17.58	 & 24.79	 & 23.17\\
GraphFormer	 & 22.53	 & 22.4	 & 22.55	 & 22.59	 & 23.07	 & 24.19	 & 17.43	 & 14.26	 & 21.59	 & 20.84 \\
\midrule
\alg	 & \textbf{34.29}	 & \textbf{37.37}	 & \textbf{38.96}	 & \textbf{36.86}	 & \textbf{38.36}	 & 55.61	 & \textbf{49.66}	 & \textbf{44.88}	 & \textbf{54.27}	 & \textbf{53.28} \\
NGAME	 & 29.18	 & 33.01	 & 35.36	 & 32.07	 & 33.9	 & \textbf{56.75}	 & 49.19	 & 44.09	 & 53.84	 & 52.41\\
DEXA	 & 29.12	 & 32.69	 & 34.86	 & 32.02	 & 33.86	 & 56.63	 & 49.05	 & 43.9	 & 53.81	 & 52.37\\
CascadeXML	 & 17.17	 & 21.7	 & 24.76	 & 19.86	 & 21.51	 & 47.82	 & 42.05	 & 38.31	 & 45.01	 & 43.77\\
XR-Transformer	 & 20.06	 & 24.85	 & 27.79	 & 23.44	 & 25.41	 & 50.14	 & 44.07	 & 39.98	 & 47.71	 & 46.59\\
PINA    & -& -& -& -&- & 55.76 & 48.70 & 43.88 &- & -\\
AttentionXML	 & 15.97	 & 19.9	 & 22.54	 & 18.23	 & 19.6	 & 45.04	 & 39.71	 & 36.25	 & 42.42	 & 41.23\\
SiameseXML	 & 27.12	 & 30.43	 & 32.52	 & 29.41	 & 30.9	 & 49.02	 & 42.72	 & 38.52	 & 46.38	 & 45.15\\
ECLARE	 & 23.43	 & 27.9	 & 30.56	 & 26.67	 & 28.61	 & 50.14	 & 44.09	 & 40	 & 47.75	 & 46.68\\
DECAF	 & 22.07	 & 26.54	 & 29.3	 & 25.06	 & 26.85	 & 50.67	 & 44.49	 & 40.35	 & 48.05	 & 46.85\\
Parabel	 & 16.94	 & 21.31	 & 24.13	 & 19.7	 & 21.34	 & 46.79	 & 41.36	 & 37.65	 & 44.39	 & 43.25\\
Bonsai	 & 18.48	 & 23.06	 & 25.95	 & 21.52	 & 23.33	 & 47.87	 & 42.19	 & 38.34	 & 45.47	 & 44.35\\
\bottomrule
    \end{tabular}
    }  
    \label{tab:results-benchmark}
\end{table*}

